On the role of resonances in polluting white dwarfs by asteroids

Pollution of white dwarf atmospheres may be caused by asteroids that originate from the locations of secular and mean-motion resonances in planetary systems. Asteroids in these locations experience increased eccentricity, leading to tidal disruption by the white dwarf. We examine how the $\nu_6$ secular resonance shifts outwards into a previously stable region of the asteroid belt, as the star evolves to a white dwarf. Analytic secular models require a planet to be engulfed in order to shift the resonance. We show with numerical simulations that as a planet gets engulfed by the evolving star, the secular resonance shifts and the rate of tidal disruption events increases with the engulfed planet's mass and its orbital separation. We also investigate the behaviour of mean-motion resonances. The width of a mean-motion resonance increases as the star loses mass and becomes a white dwarf. The $\nu_6$ secular resonance is more efficient at driving tidal disruptions than mean-motion resonances with Jupiter. By examining 230 observed exoplanetary systems whose central star will evolve into a white dwarf, we find that along with an Earth mass planet at $1\,\rm au$, hot Jupiters at a semi--major axis $a\gtrsim 0.05\,\rm au$ and super--Earths of mass $10\,\rm M_\oplus$ at $a\gtrsim 0.3\,\rm au$ represent planet types whose engulfment shifts resonances enough to cause pollution of the white dwarfs to a degree in agreement with observations.

==> RESPONSE2.tex <==
RESPONSE: We thank Dr. Alexander Mustill for refereeing the  manuscript and for the positive followup report. We have addressed all minor comments and we hope that the paper is now acceptable for publication.


Reviewer's Comments:
Reviewer: 1
Dr Alexander James Mustill
Comments to the Author
Here follows my review of MN-21-0627-MJ, "On the role of resonances in polluting white dwarfs by asteroids", by Smallwood et al.

The authors have addressed the issues I raised in my first report, and I now recommend this paper for publication. There are just a few small points of clarification and typos to be addressed:


- Abstract: "...the secular resonance shift and..." -> "resonances shift" or "resonance shifts"

RESPONSE: We have corrected the typo to "secular resonance shifts".

- Abstract, final sentence: at the moment this reads as though the engulfed planets directly cause the pollution. I'd suggest rephrasing to something like "...represent planet types whose engulfment shifts resonances enough to cause pollution...". Also, I hope the super-Earths are $10M_\oplus$ not $10M_\odot$...

RESPONSE: We have rephrased the final sentence of the abstract and also corrected the typo in the mass units of the super-Earths.

- Introduction, p1, l50: Space needed before "Around 20..."

RESPONSE: We have added a space before "Around 20". 

- Section 3.2, p8, l34: "However, by comparing the ν6 resonance gap structure after 100 Myr to the gap structure, we see..." I didn't follow this. Do you mean "...to the gap structure at t=0Myr..."?

RESPONSE: We meant comparing the gap structure of the no planet simulation with the 1 earth mass planet simulation after 100 Myr. We have now clarified this in the text. 

- Section 3.2, p8, l39: "mean-motions renounces" -> "mean-motion resonances"

RESPONSE: We  have corrected this typo. 

- Section 3.2, p8, l44: "...that white dwarf..." -> "...that white dwarf pollution..."?

RESPONSE: We have changed the sentence to include the word "pollution".

- Section 4, p10, l13: "...an engulfed $1M_\odot$ planet" -> "$M_\oplus$"

RESPONSE: We have corrected the typo in the units. 

- Section 4, p10, l40: As a caveat to the comments on Hot Jupiters: these would be engulfed very soon after the star leaves the Main Sequence, after which it takes ~10^8-10^9 years (depending on mass) to become a WD. There is therefore the risk that the new location of the secular resonance gets depleted while the star is a giant, leaving little material to survive to pollute the WD.

RESPONSE: We have made clear in section 4 that a hot Jupiter would be engulfed very soon after the star leaves the main-sequence, which may deplete the new location of the secular resonance before polluting the WD. 
